nocaps: novel object captioning at scale

Image captioning models have achieved impressive results on datasets containing limited visual concepts and large amounts of paired image-caption training data. However, if these models are to ever function in the wild, a much larger variety of visual concepts must be learned, ideally from less supervision. To encourage the development of image captioning models that can learn visual concepts from alternative data sources, such as object detection datasets, we present the first large-scale benchmark for this task. Dubbed 'nocaps', for novel object captioning at scale, our benchmark consists of 166,100 human-generated captions describing 15,100 images from the OpenImages validation and test sets. The associated training data consists of COCO image-caption pairs, plus OpenImages image-level labels and object bounding boxes. Since OpenImages contains many more classes than COCO, nearly 400 object classes seen in test images have no or very few associated training captions (hence, nocaps). We extend existing novel object captioning models to establish strong baselines for this benchmark and provide analysis to guide future work on this task.

==> figures/model_supp_pred_ex.tex <==
\begin{figure*}[!ht]
	\hspace{-0.1in}\resizebox{0.99\textwidth}{!}{
	\renewcommand{\arraystretch}{1}
	\centering
	\small
	\begin{tabularx}{\textwidth}{lXXX}
		& \multicolumn{1}{c}{\nocapsin} & \multicolumn{1}{c}{\nocapsnear} & \multicolumn{1}{c}{\nocapsout} \\
		\multicolumn{1}{l}{\textbf{Method}}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/4423bc3fc1f1ea56.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/00c5be8db0e25f5e.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/ba203a90803733a4.jpg} \\

		\cmidrule{1-4}
		\footnotesize \textbf{Up-Down}
		    & A man in a white shirt is playing baseball.
		    & A couple of men standing on top of a truck.
		    & A group of vases sitting on top of a table.\\
		\footnotesize \textbf{Up-Down + ELMo}
		    & A group of people standing around a blue table.
		    & A couple of men standing next to a truck.
		    & Two vases sitting next to each other on a table.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS}
		    & A group of people standing near a blue table.
		    & A couple of men standing on top of a \cbs{tank}.
		    & A \cbs{teapot} sitting on top of a table next to a \cbs{vase}.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS + GT}
		    & A group of people standing around a blue table.
		    & A couple of men standing on top of a \cbs{tank}.
		    & A couple of \cbs{kettle} \cbs{jugs} sitting next to each other.\\
		\midrule
		\footnotesize \textbf{NBT}
		    & A group of \nbt{men} standing in a field.
		    & A \nbt{man} standing on the back of a \nbt{tank}.
		    & A couple of \nbt{kettles} are sitting on a table.\\
		\footnotesize \textbf{NBT + CBS}
		    & A couple of \nbt{men} standing on a tennis court.
		    & A \nbt{man} standing on top of a \cbs{tank} with a truck.
		    & A close up of a \cbs{kettle} on a table.\\
		\footnotesize \textbf{NBT + CBS + GT}
		    & A group of \nbt{men} are standing in a field.
		    & A man standing on top of a \cbs{tank} \nbt{plant}.
		    & Two \cbs{kettles} and \nbt{teapot} \cbs{jugs} are sitting on a table.\\
		\midrule
		\footnotesize \textbf{Human}
		    & Two people in karate uniforms spar in front of a crowd.
		    & Two men sitting on a tank parked in the bush.
		    & Ceramic jugs are on display in a glass case.\\

		\addlinespace[0.25in]
		& \multicolumn{1}{c}{\nocapsin} & \multicolumn{1}{c}{\nocapsnear} & \multicolumn{1}{c}{\nocapsout} \\
		\multicolumn{1}{l}{\textbf{Method}}
		& \includegraphics[width=0.24\textwidth, clip]{figures/val/0b1fbd3ba02701cd.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/00f3dbbbf5bdf2cf.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/fa9c1a8fa79456a4.jpg} \\

		\cmidrule{1-4}
		\footnotesize \textbf{Up-Down}
		    & A woman riding a bike with a statue on her head.
		    & A couple of chairs sitting in front of a building.
		    & A bird sitting on the ground in the grass.\\
		\footnotesize \textbf{Up-Down + ELMo}
		    & There is a woman that is riding a bike.
		    & A room that has a lot of furniture in it.
		    & A dog laying on the ground next to a stuffed animal.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS}
		    & There is a woman that is riding a bike.
		    & Two \cbs{pillows} and a table in the \cbs{house}.
		    & A dog laying on the ground next to a \cbs{tortoise}.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS + GT}
		    & There is a woman that is riding a bike.
		    & Two \cbs{couches} and a table in a \cbs{house}.
		    & A dog laying on the ground next to a \cbs{tortoise}.\\
		\midrule
		\footnotesize \textbf{NBT}
		    & A man is riding a \nbt{clothing} on a bike.
		    & A table with a \nbt{couch} and a table.
		    & A \nbt{tortoise} is laying on top of the ground.\\
		\footnotesize \textbf{NBT + CBS}
		    & A woman is riding a \nbt{clothing} in the street.
		    & A couple of \cbs{pillows} on a wooden table in a \cbs{couch}.
		    & A \cbs{tortoise} that is sitting on the ground.\\
		\footnotesize \textbf{NBT + CBS + GT}
		    & A man is riding a \nbt{clothing} on a \nbt{person}.
		    & A \nbt{house} and a \cbs{studio couch} of \cbs{couches} in a room.
		    & A \cbs{tortoise} is laying on the ground in the grass.\\
		\midrule
		\footnotesize \textbf{Human}
            & People are performing in an open cultural dance.
            & On the deck of a pool is a couch and a display of a safety ring.
            & Three tortoises crawl on soil and wood chips in an enclosure.\\

	\end{tabularx}}
	\caption{Some challenging images from \nocaps and corresponding captions generated by existing approaches. The constraints given to the CBS are shown in \cbs{blue}. The visual words associated with NBT are shown in \nbt{red}.}
	\label{fig:pred_examples_1}
	\vspace{-10pt}
\end{figure*}

\begin{figure*}[!ht]
	\hspace{-0.1in}\resizebox{0.99\textwidth}{!}{
	\renewcommand{\arraystretch}{1}
	\centering
	\small
	\begin{tabularx}{\textwidth}{lXXX}
		& \multicolumn{1}{c}{\nocapsin} & \multicolumn{1}{c}{\nocapsnear} & \multicolumn{1}{c}{\nocapsout} \\
		\multicolumn{1}{l}{\textbf{Method}}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/05e3e00773c6c141.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/083b651122889187.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/4d1b9c4c85ad5b04.jpg}\\
        
		\cmidrule{1-4}
		\footnotesize \textbf{Up-Down}
		    & A group of people are playing a game.
		    & A large white sign on a city street.
		    & A bear laying in the grass near a tree.\\
		\footnotesize \textbf{Up-Down + ELMo}
		    & A woman in a pink dress is holding a child.
		    & A large white bus parked on the side of a road.
		    & A bear that is laying down in the grass.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS}
		    & A woman in a pink dress is holding a child.
		    & A \cbs{billboard} that has a \cbs{street light} on it.
		    & A \cbs{red panda} is walking through the grass.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS + GT}
		    & A woman in a pink dress is holding a child.
		    & A large white bus parked next to a \cbs{billboard}.
		    & A \cbs{red panda} is walking through the grass.\\
		\midrule
		\footnotesize \textbf{NBT}
		    & A group of \nbt{man} are standing in a field.
		    & A \nbt{billboard} sign on the side of a building.
		    & A brown \nbt{red panda} is laying on the grass.\\
		\footnotesize \textbf{NBT + CBS}
		    & A group of \nbt{man} are playing a baseball game.
		    & A picture of \cbs{billboard} sign on the \cbs{street light}.
		    & A \nbt{tree} and a brown \cbs{red panda} in a field.\\
		\footnotesize \textbf{NBT + CBS + GT}
		    & A group of \nbt{man} are standing on a field.
		    & A \cbs{billboard} sign on the side of a building.
		    & A brown \cbs{red panda} lying on top of a field.\\
		\midrule
		\footnotesize \textbf{Human}
		    & Two sumo wrestlers are wrestling while a crowd of men and women watch.
            & A man is standing on the ladder and working at the billboard.
            & The red panda trots across the forest floor.\\

		\addlinespace[0.25in]
		& \multicolumn{1}{c}{\nocapsin} & \multicolumn{1}{c}{\nocapsnear} & \multicolumn{1}{c}{\nocapsout} \\
		\multicolumn{1}{l}{\textbf{Method}}
	    & \includegraphics[width=0.24\textwidth, clip]{figures/val/085005e11ebacccf.jpg}
        & \includegraphics[width=0.24\textwidth, clip]{figures/val/fa9f0ce47c1a885c.jpg}
        &  \includegraphics[width=0.24\textwidth, clip]{figures/val/08633d6cdda962f2.jpg}\\
        
		\cmidrule{1-4}
		\footnotesize \textbf{Up-Down}
		    & A woman wearing a white shirt and a white shirt.
		    & A person riding a yellow bike in the field.
		    & A close up of a cat looking at a bird.\\
		\footnotesize \textbf{Up-Down + ELMo}
		    & A woman wearing a white shirt and white shirt.
		    & A woman sitting on a yellow bike.
		    & A close up of a bird with its mouth open.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS}
		    & A woman wearing a white \cbs{suit} and a white shirt.
		    & A person sitting on a bicycle with a \cbs{wheelchair}.
		    & A \cbs{sea lion} standing with its mouth open.\\
		\footnotesize \textbf{Up-Down + ELMo + CBS + GT}
		    & A woman wearing a white \cbs{suit} and a white shirt.
		    & A person sitting on a \cbs{bicycle} with a \cbs{wheelchair}.
		    & A \cbs{sea lion} standing next to a \cbs{harbor seal}.\\
		\midrule
		\footnotesize \textbf{NBT}
		    & A woman wearing a white shirt is wearing a hat.
		    & A man sitting on a \nbt{wheelchair} with a \nbt{bike}.
		    & A close up of a \nbt{sea lion} and \nbt{harbor seal} with its head.\\
		\footnotesize \textbf{NBT + CBS}
		    & A \cbs{suit} of woman wearing a white suit.
		    & A man sitting on a \cbs{wheelchair} and a \nbt{bike}.
		    & A close up of a \nbt{harbor seal} of a \cbs{sea lion}.\\
		\footnotesize \textbf{NBT + CBS + GT}
		    & A \cbs{suit} of woman wearing a white shirt.
		    & A \cbs{bicycle} sitting on a \cbs{wheelchair} with a \nbt{bike}.
		    & A close up of a \cbs{harbor seal} of a \cbs{sea lion}.\\
		\midrule
		\footnotesize \textbf{Human}
		    & The man has a wrap on his head and a white beard.
            & A person sitting in a yellow chair with wheels.
            & A brown and gray sea lion looking at the photographer. \\
	\end{tabularx}}
	\caption{Some challenging images from \nocaps and corresponding captions generated by existing approaches. The constraints given to the CBS are shown in \cbs{blue}. The visual words associated with NBT are shown in \nbt{red}.}
	\label{fig:pred_examples_1}
	\vspace{-10pt}
\end{figure*}


==> figures/nocaps_supp_example.tex <==
\begin{figure*}[h]
	\centering
	\begin{center}
	\resizebox{0.95\textwidth}{!}{
	\footnotesize
	\setlength\tabcolsep{0.5pt}
	\begin{tabularx}{\linewidth}{lXllXllX}
		\multicolumn{2}{c}{\normalsize{\nocapsin}} & ~~ & \multicolumn{2}{c}{\normalsize{\nocapsnear}} & ~~ & \multicolumn{2}{c}{\normalsize{\nocapsout}}\\
		
    \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/6e9dcdbee43b0346.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/fb71b085f783c008.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm]{figures/val/416c9c08f841f000.jpg}}\\

        1. & Two hardcover \indomain{\indomain{books}} are on the \indomain{table}  & &
            1. & \indomain{Men} in military uniforms playing instruments in an orchestra. & &
            1. & Some red invertebrate \outdomain{jellyfishes} in dark blue water. \\

        2. & Two magazines are sitting on a \indomain{coffee table}.  & &
            2. & Military officers play brass horns next to each other. & &
            2. & orange and clear \outdomain{jellyfish} in dark blue water\\

        3. & Two \indomain{\indomain{books}} and many crafting supplies are on this \indomain{table}. & &
            3. & Two \indomain{men} in camouflage clothing playing the \outdomain{trumpet}.  & &
            3. & A red \outdomain{jellyfish} is swimming around with other red \outdomain{jellyfish}.\\

        4. & a recipe \indomain{book} and sewing \indomain{book} on a craft \indomain{table} & &
            4. & Two \indomain{men} dressed in military outfits play the french horn. & &
            4. & Orange \outdomain{jellyfish} swimming through the water. \\

        5. & Two hardcover \indomain{\indomain{books}} are laying on a \indomain{table}. & &
            5. & Two \indomain{people} dressed in camoflauge uniforms playing musical instruments. & &
            5. & Bright orange and clear \outdomain{jellyfish} swim in open water.\\

        6. & A \indomain{table} with two different \indomain{\indomain{books}} on it. & &
            6. & A couple \indomain{people} in uniforms holding tubas by their mouths. & &
            6. & The fish is going through the very blue water.\\

        7. & Two different \indomain{books} on sewing and cooking/baking on a \indomain{table}. & &
            7. & Two \indomain{people} in uniform are playing the tuba. & &
            7. & A bright orange \outdomain{jellyfish} floating in the water.\\

        8. & Two magazine \indomain{books} are sitting on a \indomain{table} with arts and craft materials. & &
            8. & A couple of military \indomain{men} playing the french horn.  & &
            8. & Several red \outdomain{jellyfish} swimming in bright blue water.\\

        9. & A couple of \indomain{books} are on a \indomain{table}. & &
            9. & A \indomain{man} in uniform plays a French horn. & &
            9. & An orange \outdomain{jellyfish} swimming with a blue background\\

        10. & The \indomain{person} is there looking into the \indomain{book}. & &
            10. & Two \indomain{men} are playing the \outdomain{trumpet} standing nearby. & &
            10. & A very vibrantly red \outdomain{jellyfish} is seen swimming in the water.\\
            \addlinespace[0.1cm]
        \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm]{figures/val/2c4004388f263f72.jpg}} 
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/f89f1c0793c6947f.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/0b5547d4aa16e365.jpg}}\\


        1. & Jockeys on \indomain{horses} racing around a track.  & &
            1. & Two \indomain{people} in a fencing match with a \indomain{woman} walking by in the background. & &
            1. & A \outdomain{panda} bear sitting beside a smaller \outdomain{panda} bear.\\

        2. & Several \indomain{horses} are running in a race thru the grass. & &
            2. & Two \indomain{people} in masks fencing with each other. & &
            2. & The \outdomain{panda} is large and standing over the plant.\\
        3. & several \indomain{people} racing \indomain{horses} around a turn outside & &
            3. & Two \indomain{people} in white garbs are fencing while \indomain{people} watch. & &
            3. & Two \outdomain{panda} are eating sticks from plants. \\
        4. & Uniformed jockeys on \indomain{horses} racing through a grass field. & &
            4. & Two \indomain{people} in full gear fencing on white mat. & &
            4. & Two \outdomain{panda} bears sitting with greenery surrounding them.\\
        5. & Several \indomain{horse} jockies are riding \indomain{horses} around a turn. & &
            5. & A couple of \indomain{people} in white outfits are fencing. & &
            5. & two \outdomain{panda} bears in the bushes eating bamboo sticks \\
        6. & Six men and six \indomain{horses} are racing outside & &
            6. & Two fencers in white outfits are dueling indoors. & &
            6. & two \outdomain{pandas} sitting in the grass eating some plants\\
        7. & A group of men wearing sunglasses and racing on a horse  & &
            7. & A couple of \indomain{people} doing a fencing competition inside.  & &
            7. & two \outdomain{pandas} are eating a green leaf from a plant\\
        8. & Six \indomain{horses} with riders are racing, leaning over at an incredible angle. & &
            8. & Two \indomain{people} in white clothes fencing each other. & &
            8. & Two \outdomain{pandas} are eating bamboo in a wooded area.\\

        9. & Seveal \indomain{people} wearing goggles and helmets racing \indomain{horses}. & &
            9. & Two \indomain{people} in an room competing in a fencing competition. & &
            9. & \outdomain{Pandas} enjoy the outside and especially with a friend.\\

        10. & a row of \indomain{horses} and jockeys running in the same direction in a line & &
            10. & Two \indomain{people} in all white holding swords and fencing. & &
            10. & Two black and white \outdomain{panda} bears eating leaf stems \\
	\end{tabularx}}
	\end{center}\vspace{-10pt}
	\caption{Examples of images belonging to the \nocapsin, \nocapsnear and \nocapsout subsets of the \nocaps validation set. Each image is annotated with 10 reference captions, capturing more of the salient content of the image and improving the accuracy of automatic evaluations~\cite{Vedantam2015,spice2016}. Categories in \indomain{orange} are \nocapsin object classes while categories in \outdomain{blue} are \nocapsout classes. Note that not all captions mention the ground-truth object classes consistent with the instructions provided on the data collection interface.}
	\label{fig:examples1}
	\vspace{-15pt}
\end{figure*}

\begin{figure*}[t!]
	\centering
	\begin{center}
	\resizebox{0.95\textwidth}{!}{
	\footnotesize
	\setlength\tabcolsep{0.5pt}
	\begin{tabularx}{\linewidth}{lXllXllX}
		\multicolumn{2}{c}{\normalsize{\nocapsin}} & ~~ & \multicolumn{2}{c}{\normalsize{\nocapsnear}} & ~~ & \multicolumn{2}{c}{\normalsize{\nocapsout}}\\
		
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/04ccb05e32dc45de.jpg}} 
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/c6fa0a8fcd9961f1.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/2feba53355b4e765.jpg}}\\


        1. & A \indomain{dog} sitting beside a \indomain{man} walking on the lawn  & &
            1. & A \indomain{woman} is sitting  with a \outdomain{camera} in front of her & &
            1. & Some decorations are have red lights you can see at night.\\

        2. & A small \indomain{dog} looking up at a \indomain{person} standing next to him. & &
            2. & A beautiful brown haired \indomain{woman} next to a \outdomain{camera}. & &
            2. & A couple of red \outdomain{lanterns} floating in the air.\\

        3. & A young \indomain{dog} looks up at their owner. & &
            3. & A \indomain{woman} poses to take a picture in a mirror. & &
            3. & Many red Chinese \outdomain{lanterns} are hung outside at night\\

        4. & A little puppy looking up at a \indomain{person}.  & &
            4. & A \indomain{women} with brown hair holding a \outdomain{camera}. & &
            4. & Floating lighted \outdomain{lanterns} on a dark night in the city. \\

        5. & A \indomain{dog} sitting on the grass next to a human. & &
            5. & A \indomain{woman} behind a \outdomain{camera} on a \outdomain{tripod}. & &
            5. & Dozens of glowing paper \outdomain{lanterns} floating off into the sky.\\

        6. & A \indomain{dog} is looking up at the \indomain{person} who is wearing jeans.   & &
            6. & A \indomain{woman} sits with her head leaned behind a \outdomain{camera}. & &
            6. & A black night sky with red, bright floating \outdomain{lanterns}.\\

        7. & The tan \indomain{dog} sits patiently beside the \indomain{person}.l & &
            7. & A girl looking pity behind a \outdomain{camera} on a \outdomain{tripod}. & &
            7. & Red \outdomain{lanterns} floating up to the dark night sky.\\

        8. & The white \indomain{dog} is sitting in the grass by a \indomain{person} who is standing up.   & &
            8. & A \indomain{woman} sits and tilts her head while behind a \outdomain{camera}. & &
            8. & Chinese \outdomain{lanterns} that are red are floating into the sky.\\

        9. & The tan \indomain{dog} happily accompanies the human on the grass. & &
            9. & A \indomain{woman} is sitting behind a \outdomain{camera} with \outdomain{tripod}.  & &
            9. & This town has many lit Chinese \outdomain{lanterns} hanging between the buildings.\\

        10. & A \indomain{dog} is on the grass is looking to a \indomain{person} & &
            10. & A \indomain{woman} with a \outdomain{camera} in front of her. & &
            10. & The street is filled with light from hanging \outdomain{lanterns}.\\
        \addlinespace[0.2cm]
        \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/e2d6553151f7231b.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/eccb080e57b2aac5.jpg}}
            & 
            & 
            \multicolumn{2}{c}{\includegraphics[width=0.33\linewidth,height=4cm, clip]{figures/val/740fc2fafd5b3c63.jpg}}\\


        1. & \indomain{people} are standing on the side of a food \indomain{truck}  & &
            1. & A room with a hot tub and sauna.  & &
            1. & Large silver \outdomain{tanks} behind the counter at a restaurant. \\

        2. & A food \indomain{truck} parked with \indomain{people} standing in line.  & &
            2. & A white hot tub is next to some wood. & &
            2. & Shiny metal \outdomain{containers} with writing are beside each other.\\

        3. & \indomain{people} standing outside and ordering from a food \indomain{truck} in the daytime. & &
            3. & A \outdomain{jacuzzi} sitting on rocks inside of a patio. & &
            3. & A brewery with big, silver, metal \outdomain{containers} and a sign.\\

        4. & The food \indomain{truck} has a line of \indomain{people} in front of the window. & &
            4. & A hot tub sits in the middle of the room. & &
            4. & A brew station inside of a restaurant. \\

        5. & A \indomain{woman} standing in front of a food \indomain{truck}. & &
            5. & A \outdomain{jacuzzi} sitting near some rocks and a sauna & &
            5. & Large steel breweries sit behind a chalkboard displaying different food and drink deals.\\

        6. & A food  \indomain{truck} outside of a small business  with several \indomain{people} eating  & &
            6. & A hot tub in a room with wooden flooring. & &
            6. & A cabinetry with big tin cans and a chalkboard on the top\\

        7. & \indomain{people} stand in line to get food from a food \indomain{truck}. & &
            7. & A room is shown with a hot tub, decorative plants and some paintings ont he wall. & &
            7. & A man works on machinery inside a brewery.\\

        8. & A large metal \indomain{truck} serving food to \indomain{people} in a parking lot. & &
            8. & A room with a large hot tub and a sauna. & &
            8. & The many silver \outdomain{tanks} are used for beverage making.\\

        9. & \indomain{men} and \indomain{women} speaking in front of a grey food \indomain{truck} that is open for business. & &
            9. & A water filled \outdomain{jacuzzi} surrounded by smooth river rocks and a wooden deck. & &
            9. & A menu is hanging above a craft brewery.\\

        10. & \indomain{woman} wearing jeans in front of the \indomain{truck} & &
            10. & A white and grey \outdomain{jacuzzi} around rock building  & &
            10. & A man peers at a brewing tank while standing on a step ladder. \\
	\end{tabularx}}
	\end{center}\vspace{-10pt}
	\caption{More examples of images belonging to the \nocapsin, \nocapsnear and \nocapsout subsets of the \nocaps validation set. Each image is annotated with 10 reference captions, capturing more of the salient content of the image and improving the accuracy of automatic evaluations~\cite{Vedantam2015,spice2016}. Categories in \indomain{orange} are \nocapsin object classes while categories in \outdomain{blue} are \nocapsout classes. Note that not all captions mention the ground-truth object classes consistent with the instructions provided on the data collection interface.}
	\label{fig:examples2}
	\vspace{-15pt}
\end{figure*}


